Eidos: Efficient, Imperceptible Adversarial 3D Point Clouds

Classification of 3D point clouds is a challenging machine learning (ML) task with important real-world applications in a spectrum from autonomous driving and robot-assisted surgery to earth observation from low orbit. As with other ML tasks, classification models are notoriously brittle in the presence of adversarial attacks. These are rooted in imperceptible changes to inputs with the effect that a seemingly well-trained model ends up misclassifying the input. This paper adds to the understanding of adversarial attacks by presenting Eidos, a framework providing Efficient Imperceptible aDversarial attacks on 3D pOint cloudS. Eidos supports a diverse set of imperceptibility metrics. It employs an iterative, two-step procedure to identify optimal adversarial examples, thereby enabling a runtime-imperceptibility trade-off. We provide empirical evidence relative to several popular 3D point cloud classification models and several established 3D attack methods, showing Eidos' superiority with respect to efficiency as well as imperceptibility.

==> tex/baseline-report.tex <==
\begin{table}[h!]
    \centering
    \caption{Si-adv white-box attack}
    
    \resizebox{\linewidth}{!}{
        \begin{tabular}{m{2.5cm} p{1.5cm} p{1.8cm} p{1.8cm} p{1.8cm} p{1.8cm}}
        \hline
         Victim model & PointNet & PointNet++ & DGCNN \\
         \hline
         A.S.R & 0.997 & 0.990 & 0.998 \\
         MSE & 0.580 & 0.941 & 0.993 \\
         C.D ($10^{-4}$) & 2.146 & 5.647 & 6.358  \\
         H.D ($10^{-2}$) & 2.045 & 1.877 & 1.278  \\
         A.T (s) & 41.33 & 446.95 & 132.00  \\
     \hline
    \end{tabular}
    }
    \label{tab:table1}
\end{table}




% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table*}[h!]\tiny
\centering
\caption{Si-adv Black-box transfer-based attack}
\begin{tabular}{@{}lllllllllllllll@{}}
\toprule
\multicolumn{1}{c}{\multirow{3}{*}{\textbf{Attack}}} & \multicolumn{4}{c}{\textbf{PointNet}}                   &  & \multicolumn{4}{c}{\textbf{PointNet++}}                 &  & \multicolumn{4}{c}{\textbf{dsgnn}}                      \\ \cmidrule(lr){2-5} \cmidrule(lr){7-10} \cmidrule(l){12-15} 
\multicolumn{1}{c}{}                                 & \textbf{ASR} & \textbf{MSE} & \textbf{CD} & \textbf{HD} &  & \textbf{ASR} & \textbf{MSE} & \textbf{CD} & \textbf{HD} &  & \textbf{ASR} & \textbf{MSE} & \textbf{CD} & \textbf{HD} \\
\multicolumn{1}{c}{}                                 & (\%)         &              & ($10^{-4}$)        & ($10^{-2}$)        &  & (\%)         &              & ($10^{-4}$)        & ($10^{-2}$)        &  & (\%)         &              & ($10^{-4}$)        & ($10^{-2}$)        \\
\textbf{PointNet}                                    & 99.8              & 0.58             & 2.14            & 2.05            &  & 17.9         & 0.94         & 5.67        & 1.86             &  & 9.3         & 0.99         & 6.33        & 1.27             \\
\textbf{PointNet++}                                  & 12.6         & 0.58         & 2.15        & 2.04         &  & 99.1         & 0.94         & 5.65        & 1.88        &  & 18.2             & 0.94             & 5.61            & 1.85            \\
\textbf{dsgnn}                                       & 13.7         & 0.58         & 2.15        & 2.04             &  & 18.2             & 0.94             & 5.61            & 1.85            &  & 99.8             &    0.99          & 6.36            & 1.28            \\ \bottomrule
\end{tabular}
\end{table*}


\begin{table}[h!]
    \centering
    \caption{$GeoA^3$ white-box attack}
    
    \resizebox{\linewidth}{!}{
        \begin{tabular}{m{2.5cm} p{1.5cm} p{1.8cm} p{1.8cm} p{1.8cm} p{1.8cm}}
        \hline
         Victim model & PointNet & PointNet++ & DGCNN \\
         \hline
         A.S.R & 1.00 & 1.00 & N/A \\
         MSE & N/A & N/A & N/A \\
         C.D ($10^{-4}$) & 12.5 & 35.2 & N/A  \\
         H.D ($10^{-2}$) & 0.22 & 1.58 & N/A  \\
         Cur ($10^{-4}$) & 7.66 & 49.00 & N/A  \\
         A.T (s) & N/A & N/A & N/A  \\
     \hline
    \end{tabular}
    }
    \label{tab:table1}
\end{table}

\begin{table}[h!]
    \centering
    \caption{Mesh-Attack white-box attack}
    
    \resizebox{\linewidth}{!}{
        \begin{tabular}{m{2.5cm} p{1.5cm} p{1.8cm} p{1.8cm} p{1.8cm} p{1.8cm}}
        \hline
         Victim model & PointNet & PointNet++ & DGCNN \\
         \hline
         A.S.R & N/A & N/A & N/A \\
         MSE & N/A & N/A & N/A \\
         C.D ($10^{-4}$) & N/A & N/A & N/A  \\
         H.D ($10^{-2}$) & N/A & N/A & N/A  \\
         A.T (s) & N/A & N/A & N/A  \\
     \hline
    \end{tabular}
    }
    \label{tab:table1}
\end{table}


\begin{table}[h!]
    \centering
    \caption{Attack on PointNet over ModelNet40 }
    
    \resizebox{\linewidth}{!}{
        \begin{tabular}{m{2.5cm} p{1.5cm} p{1.8cm} p{1.8cm} p{1.8cm} p{1.8cm}}
        \hline
         Attacker & SI-adv & Geoa$^3$ & advPC & GSDA \\
         \hline
         A.S.R & 0.996 & \textbf{1.000} & 0.922 & 0.998 \\
         L2 & 0.648 & 7.754 & \textbf{0.582} & 9.208 \\
         C.D ($10^{-4}$) & \textbf{3.081} & 3.408 & 4.237 & 3.348  \\
         H.D ($10^{-2}$) & 4.246 & \textbf{0.184} & 1.595 & 0.399 \\
         Curv ($10^{-2}$) & 0.271 & \textbf{0.187} & 1.076 & 0.219\\
         Smooth ($10^{-2}$) & \textbf{0.120} & 0.187 & 0.158 & 0.180\\
         A.T (s) & \textbf{0.828} & 76.25 & 14.76 & 63.37 \\
     \hline
    \end{tabular}
    }
    \label{tab:table1}
\end{table}


\begin{table}[h!]
    \centering
    \caption{Attack on PointNet over ModelNet40 by SI-ADV}
    
    \resizebox{\linewidth}{!}{
        \begin{tabular}{m{2.5cm} p{1.5cm} p{1.5cm} p{1.5cm} p{1.5cm} p{1.5cm} p{1.5cm} p{1.5cm}}
        \hline
         Attacker & Vanilla & Adam & BP@L2 & BP@Curv & BP@HD & BP@CD &SIBP@L2  \\
         \hline
         A.S.R & 0.996 & \textbf{0.998} & 0.996 & 0.996 & 0.996 & 0.996 & 0.996\\
         L2 & 0.648 & 0.752 & \textbf{0.108} & 0.565 & 0.149 & 0.595 & 0.228\\
         C.D ($10^{-4}$) & 3.081 & 3.681 & \textbf{0.953} & 2.755 & 0.978 & 2.893 & 1.631\\
         H.D ($10^{-2}$) & 4.246 & 4.211 & 2.432 & 3.787 & \textbf{1.700} & 4.871 & 6.667\\
         Curv ($10^{-2}$) & 0.271 & 0.316 & 0.193 & 0.249 & 0.193 & 0.269 & \textbf{0.105}\\
         Smooth ($10^{-2}$) & \textbf{0.120} & 0.123 & 0.136 & 0.125 & 0.144 & 0.123 & \textbf{0.105}\\
         A.T (s) & \textbf{0.828} & \textbf{0.802} & \textbf{0.503} & \textbf{0.623} & \textbf{0.533} & \textbf{0.535} & \textbf{0.569}\\
     \hline
    \end{tabular}
    }
    \label{tab:table1}
\end{table}

\begin{table}[h!]
    \centering
    \caption{Attack on PointNet over ModelNet40 by SI-ADV}
    
    \resizebox{\linewidth}{!}{
        \begin{tabular}{m{2.5cm} p{1.5cm} p{1.5cm} p{1.5cm} p{2.0cm} p{2.0cm}}
        \hline
         Attacker & Vanilla Step50 & BP@L2 Step50  &SIBP@L2 Step50 & BP@L2 Step100 & SIBP@L2 Step100  \\
         \hline
         A.S.R & 0.996 & 0.996 & 0.996 & \textbf{1.000} & \textbf{1.000}\\
         L2 & 0.648 & 0.108 & 0.228 & \textbf{0.094} & 0.194\\
         C.D ($10^{-4}$) & 3.081 & 0.953 & 1.631 & \textbf{0.861} & 1.477\\
         H.D ($10^{-2}$) & 4.246 & 2.432 & 6.667 & \textbf{2.251} & 6.239  \\
         Curv ($10^{-2}$) & 0.271 & 0.136 & 0.105 & 0.181 & \textbf{0.100} \\
         Smooth ($10^{-2}$) & 0.120 & 0.136 & 0.105 & 0.138 & \textbf{0.106}\\
     \hline
    \end{tabular}
    }
    \label{tab:table1}
\end{table}
\begin{table}[h!]
    \centering
    \caption{Attack on PointNet over ModelNet40 by SI-ADV}
    
    \resizebox{\linewidth}{!}{
        \begin{tabular}{m{2.5cm} p{1.5cm} p{1.5cm} p{1.5cm} p{2.0cm} p{2.0cm}}
        \hline
         Attacker & Vanilla & BP@L2 & SIBP@L2 & BP2@L2 & SIBP2@L2\\
         \hline
         A.S.R & 0.996 & \textbf{1.000} & \textbf{1.000}& \textbf{1.000}& \textbf{1.000} \\
         L2 & 0.648 & 0.094 & 0.194 & \textbf{0.071} & 0.264\\
         C.D ($10^{-4}$) & 3.081 & 0.861 & 1.477 & \textbf{0.607} & 1.608\\
         H.D ($10^{-2}$) & 4.246 & 2.251 & 6.239 & \textbf{1.366} & 2.893 \\
         Curv ($10^{-2}$) & 0.271 &  0.181 & \textbf{0.100} & 0.114 & 0.167\\
         Smooth ($10^{-2}$) & 0.120 &  0.138 & \textbf{0.106} & 0.148 & 0.126 \\
     \hline
    \end{tabular}
    }
    \label{tab:table1}
\end{table}

\begin{table}[h!]
    \centering
    \caption{Attack on PointNet over ModelNet40 }
    
    \resizebox{\linewidth}{!}{
        \begin{tabular}{m{2.5cm} p{1.5cm} p{1.8cm} p{1.8cm} p{1.8cm} p{1.8cm} p{1.8cm}}
        \hline
         Attacker & SI-adv & Geoa$^3$ & advPC & GSDA & GSDA@BP3L2HD\\
         \hline
         A.S.R & 0.996 & \textbf{1.000} & 0.922 & 0.998 & 1.000 \\
         L2 & 0.648 & 7.754 & \textbf{0.582} & 9.208 & 0.243 \\
         C.D ($10^{-4}$) & \textbf{3.081} & 3.408 & 4.237 & 3.348 & 1.519 \\
         H.D ($10^{-2}$) & 4.246 & \textbf{0.184} & 1.595 & 0.399 & 0.735 \\
         Curv ($10^{-2}$) & 0.271 & \textbf{0.187} & 1.076 & 0.219 & 0.357 \\
         Smooth ($10^{-2}$) & \textbf{0.120} & 0.187 & 0.158 & 0.180 & 0.169 \\
         A.T (s) & \textbf{0.828} & 76.25 & 14.76 & 63.37 & 12.10 \\
     \hline
    \end{tabular}
    }
    \label{tab:table1}
\end{table}

==> tex/bib.tex <==
\begin{thebibliography}{41}
% \providecommand{\natexlab}[1]{#1}
% \providecommand{\url}[1]{\texttt{#1}}
% \expandafter\ifx\csname urlstyle\endcsname\relax
%   \providecommand{\doi}[1]{doi: #1}\else
%   \providecommand{\doi}{doi: \begingroup \urlstyle{rm}\Url}\fi

\bibitem[Singh et~al.(2019)Singh, Mittal, and Bhatia]{singh20193d}
Rahul~Dev Singh, Ajay Mittal, and Rajesh~K Bhatia.
\newblock 3d convolutional neural network for object recognition: a review.
\newblock \emph{Multimedia Tools and Applications}, 78:\penalty0 15951--15995, 2019.

\bibitem[Maturana and Scherer(2015)]{maturana2015voxnet}
Daniel Maturana and Sebastian Scherer.
\newblock Voxnet: A 3d convolutional neural network for real-time object recognition.
\newblock In \emph{2015 IEEE/RSJ international conference on intelligent robots and systems (IROS)}, pages 922--928. IEEE, 2015.

\bibitem[Qi et~al.(2017{\natexlab{a}})Qi, Su, Mo, and Guibas]{pointnet}
Charles~R Qi, Hao Su, Kaichun Mo, and Leonidas~J Guibas.
\newblock Pointnet: Deep learning on point sets for 3d classification and segmentation.
\newblock In \emph{Proceedings of the IEEE conference on computer vision and pattern recognition}, pages 652--660, 2017{\natexlab{a}}.

\bibitem[Qi et~al.(2017{\natexlab{b}})Qi, Yi, Su, and Guibas]{pointnet++}
Charles~Ruizhongtai Qi, Li~Yi, Hao Su, and Leonidas~J Guibas.
\newblock Pointnet++: Deep hierarchical feature learning on point sets in a metric space.
\newblock \emph{Advances in neural information processing systems}, 30, 2017{\natexlab{b}}.

\bibitem[Duan et~al.(2019)Duan, Zheng, Lu, Zhou, and Tian]{8953340}
Yueqi Duan, Yu~Zheng, Jiwen Lu, Jie Zhou, and Qi~Tian.
\newblock Structural relational reasoning of point clouds.
\newblock In \emph{2019 IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR)}, pages 949--958, 2019.
\newblock \doi{10.1109/CVPR.2019.00104}.

\bibitem[Liu et~al.(2019{\natexlab{a}})Liu, Fan, Meng, Lu, Xiang, and Pan]{Densepoint}
Yongcheng Liu, Bin Fan, Gaofeng Meng, Jiwen Lu, Shiming Xiang, and Chunhong Pan.
\newblock Densepoint: Learning densely contextual representation for efficient point cloud processing.
\newblock In \emph{Proceedings of the IEEE/CVF international conference on computer vision}, pages 5239--5248, 2019{\natexlab{a}}.

\bibitem[Yang et~al.(2019{\natexlab{a}})Yang, Zhang, Ni, Li, Liu, Zhou, and Tian]{yang2019modeling}
Jiancheng Yang, Qiang Zhang, Bingbing Ni, Linguo Li, Jinxian Liu, Mengdie Zhou, and Qi~Tian.
\newblock Modeling point clouds with self-attention and gumbel subset sampling.
\newblock In \emph{Proceedings of the IEEE/CVF conference on computer vision and pattern recognition}, pages 3323--3332, 2019{\natexlab{a}}.

\bibitem[EU(2023)]{AIAct}
EU.
\newblock The artificial intelligence act, 2023.
\newblock [Online] https://artificialintelligenceact.eu.

\bibitem[Liu et~al.(2019{\natexlab{b}})Liu, Yu, and Su]{liu2019extending}
Daniel Liu, Ronald Yu, and Hao Su.
\newblock Extending adversarial attacks and defenses to deep 3d point cloud classifiers.
\newblock In \emph{2019 IEEE International Conference on Image Processing (ICIP)}, pages 2279--2283. IEEE, 2019{\natexlab{b}}.

\bibitem[Wen et~al.(2019)Wen, Lin, Chen, Chen, and Jia]{geoa3}
Yuxin Wen, Jiehong Lin, Ke~Chen, CL~Chen, and Kui Jia.
\newblock Geometry-aware generation of adversarial point clouds.
\newblock \emph{arXiv preprint arXiv:1912.11171}, 2019.

\bibitem[Zhou et~al.(2020)Zhou, Chen, Liao, Chen, Dong, Liu, Zhang, Hua, and Yu]{zhou2020lg}
Hang Zhou, Dongdong Chen, Jing Liao, Kejiang Chen, Xiaoyi Dong, Kunlin Liu, Weiming Zhang, Gang Hua, and Nenghai Yu.
\newblock Lg-gan: Label guided adversarial network for flexible targeted attack of point cloud based deep networks.
\newblock In \emph{Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition}, pages 10356--10365, 2020.

\bibitem[Huang et~al.(2022)Huang, Dong, Chen, Zhou, Zhang, and Yu]{si_adv_pc}
Qidong Huang, Xiaoyi Dong, Dongdong Chen, Hang Zhou, Weiming Zhang, and Nenghai Yu.
\newblock Shape-invariant 3d adversarial point clouds.
\newblock In \emph{Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition}, pages 15335--15344, 2022.

\bibitem[Hu et~al.(2022)Hu, Liu, and Hu]{gsda}
Qianjiang Hu, Daizong Liu, and Wei Hu.
\newblock Exploring the devil in graph spectral domain for 3d point cloud attacks.
\newblock \emph{arXiv preprint arXiv:2202.07261}, 2022.

\bibitem[Zhang et~al.(2020{\natexlab{a}})Zhang, Avrithis, Furon, and Amsaleg]{zhang2020walking}
Hanwei Zhang, Yannis Avrithis, Teddy Furon, and Laurent Amsaleg.
\newblock Walking on the edge: Fast, low-distortion adversarial examples.
\newblock \emph{IEEE Transactions on Information Forensics and Security}, 16:\penalty0 701--713, 2020{\natexlab{a}}.

\bibitem[Xiang et~al.(2019)Xiang, Qi, and Li]{origin}
Chong Xiang, Charles~R Qi, and Bo~Li.
\newblock Generating 3d adversarial point clouds.
\newblock In \emph{Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition}, pages 9136--9144, 2019.

\bibitem[Tsai et~al.(2020)Tsai, Yang, Ho, and Jin]{tsai2020robust}
Tzungyu Tsai, Kaichen Yang, Tsung-Yi Ho, and Yier Jin.
\newblock Robust adversarial objects against deep learning models.
\newblock In \emph{Proceedings of the AAAI Conference on Artificial Intelligence}, volume~34, pages 954--962, 2020.

\bibitem[Wang et~al.(2004)Wang, Bovik, Sheikh, and Simoncelli]{wang2004image}
Zhou Wang, Alan~C Bovik, Hamid~R Sheikh, and Eero~P Simoncelli.
\newblock Image quality assessment: from error visibility to structural similarity.
\newblock \emph{IEEE transactions on image processing}, 13\penalty0 (4):\penalty0 600--612, 2004.

\bibitem[Hamdi et~al.(2020)Hamdi, Rojas, Thabet, and Ghanem]{hamdi2020advpc}
Abdullah Hamdi, Sara Rojas, Ali Thabet, and Bernard Ghanem.
\newblock Advpc: Transferable adversarial perturbations on 3d point clouds.
\newblock In \emph{Computer Vision--ECCV 2020: 16th European Conference, Glasgow, UK, August 23--28, 2020, Proceedings, Part XII 16}, pages 241--257. Springer, 2020.

\bibitem[Yang et~al.(2019{\natexlab{b}})Yang, Zhang, Fang, Ni, Liu, and Tian]{yang2019adversarial}
Jiancheng Yang, Qiang Zhang, Rongyao Fang, Bingbing Ni, Jinxian Liu, and Qi~Tian.
\newblock Adversarial attack and defense on point sets.
\newblock \emph{arXiv preprint arXiv:1902.10899}, 2019{\natexlab{b}}.

\bibitem[Kim et~al.(2021)Kim, Hua, Nguyen, and Yeung]{kim2021minimal}
Jaeyeon Kim, Binh-Son Hua, Thanh Nguyen, and Sai-Kit Yeung.
\newblock Minimal adversarial examples for deep learning on 3d point clouds.
\newblock In \emph{Proceedings of the IEEE/CVF International Conference on Computer Vision}, pages 7797--7806, 2021.

\bibitem[Shi et~al.(2022)Shi, Chen, Xu, Yang, Yu, and Huang]{shi2022shape}
Zhenbo Shi, Zhi Chen, Zhenbo Xu, Wei Yang, Zhidong Yu, and Liusheng Huang.
\newblock Shape prior guided attack: Sparser perturbations on 3d point clouds.
\newblock In \emph{Proceedings of the AAAI Conference on Artificial Intelligence}, volume~36, pages 8277--8285, 2022.

\bibitem[Goodfellow et~al.(2014)Goodfellow, Shlens, and Szegedy]{goodfellow2014explaining}
Ian~J Goodfellow, Jonathon Shlens, and Christian Szegedy.
\newblock Explaining and harnessing adversarial examples.
\newblock \emph{arXiv:1412.6572}, 2014.

\bibitem[Kurakin et~al.(2016)Kurakin, Goodfellow, and Bengio]{kurakin2016physical}
Alexey Kurakin, Ian Goodfellow, and Samy Bengio.
\newblock Adversarial examples in the physical world.
\newblock \emph{arXiv:1607.02533}, 2016.

\bibitem[Papernot et~al.(2016)Papernot, McDaniel, Jha, Fredrikson, Celik, and Swami]{papernot2016limitations}
Nicolas Papernot, Patrick McDaniel, Somesh Jha, Matt Fredrikson, Z~Berkay Celik, and Ananthram Swami.
\newblock The limitations of deep learning in adversarial settings.
\newblock In \emph{2016 IEEE European symposium on security and privacy (EuroS\&P)}, pages 372--387. IEEE, 2016.

\bibitem[Zheng et~al.(2019)Zheng, Chen, Yuan, Li, and Ren]{zheng2019pointcloud}
Tianhang Zheng, Changyou Chen, Junsong Yuan, Bo~Li, and Kui Ren.
\newblock Pointcloud saliency maps.
\newblock In \emph{Proceedings of the IEEE/CVF International Conference on Computer Vision}, pages 1598--1606, 2019.

\bibitem[Wicker and Kwiatkowska(2019)]{wicker2019robustness}
Matthew Wicker and Marta Kwiatkowska.
\newblock Robustness of 3d deep learning in an adversarial setting.
\newblock In \emph{Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition}, pages 11767--11775, 2019.

\bibitem[Zheng et~al.(2018)Zheng, Chen, Ren, et~al.]{zheng2018learning}
Tianhang Zheng, Changyou Chen, Kui Ren, et~al.
\newblock Learning saliency maps for adversarial point-cloud generation.
\newblock \emph{arXiv preprint arXiv:1812.01687}, 2018.

\bibitem[Liu et~al.(2020)Liu, Yu, and Su]{liu2020adversarial}
Daniel Liu, Ronald Yu, and Hao Su.
\newblock Adversarial shape perturbations on 3d point clouds.
\newblock In \emph{Computer Vision--ECCV 2020 Workshops: Glasgow, UK, August 23--28, 2020, Proceedings, Part I 16}, pages 88--104. Springer, 2020.

\bibitem[Zhang et~al.(2021)Zhang, Chen, Liu, Ouyang, Xie, Zhu, Li, and Meng]{mesh-attack}
Jinlai Zhang, Lyujie Chen, Binbin Liu, Bo~Ouyang, Qizhi Xie, Jihong Zhu, Weiming Li, and Yanmei Meng.
\newblock 3d adversarial attacks beyond point cloud.
\newblock \emph{arXiv preprint arXiv:2104.12146}, 2021.

\bibitem[Miao et~al.(2022)Miao, Dong, Zhu, and Gao]{miao2022isometric}
Yibo Miao, Yinpeng Dong, Jun Zhu, and Xiao-Shan Gao.
\newblock Isometric 3d adversarial examples in the physical world.
\newblock \emph{arXiv preprint arXiv:2210.15291}, 2022.

\bibitem[Carlini and Wagner(2017)]{carlini2017towards}
Nicholas Carlini and David Wagner.
\newblock Towards evaluating the robustness of neural networks.
\newblock In \emph{2017 ieee symposium on security and privacy (sp)}, pages 39--57. Ieee, 2017.

\bibitem[Tang et~al.(2022{\natexlab{a}})Tang, Shi, Wu, Peng, Khan, Zhu, and Gu]{tang2022normalattack}
Keke Tang, Yawen Shi, Jianpeng Wu, Weilong Peng, Asad Khan, Peican Zhu, and Zhaoquan Gu.
\newblock Normalattack: Curvature-aware shape deformation along normals for imperceptible point cloud attack.
\newblock \emph{Security and Communication Networks}, 2022, 2022{\natexlab{a}}.

\bibitem[Tang et~al.(2022{\natexlab{b}})Tang, Shi, Lou, Peng, He, Zhu, Gu, and Tian]{tang2022rethinking}
Keke Tang, Yawen Shi, Tianrui Lou, Weilong Peng, Xu~He, Peican Zhu, Zhaoquan Gu, and Zhihong Tian.
\newblock Rethinking perturbation directions for imperceptible adversarial attacks on point clouds.
\newblock \emph{IEEE Internet of Things Journal}, 2022{\natexlab{b}}.

\bibitem[Wu et~al.(2015)Wu, Song, Khosla, Yu, Zhang, Tang, and Xiao]{wu20153d}
Zhirong Wu, Shuran Song, Aditya Khosla, Fisher Yu, Linguang Zhang, Xiaoou Tang, and Jianxiong Xiao.
\newblock 3d shapenets: A deep representation for volumetric shapes.
\newblock In \emph{Proceedings of the IEEE conference on computer vision and pattern recognition}, pages 1912--1920, 2015.

\bibitem[Wang et~al.(2019)Wang, Sun, Liu, Sarma, Bronstein, and Solomon]{dgcnn}
Yue Wang, Yongbin Sun, Ziwei Liu, Sanjay~E Sarma, Michael~M Bronstein, and Justin~M Solomon.
\newblock Dynamic graph cnn for learning on point clouds.
\newblock \emph{Acm Transactions On Graphics (tog)}, 38\penalty0 (5):\penalty0 1--12, 2019.

\bibitem[Zhang et~al.(2020{\natexlab{b}})Zhang, Avrithis, Furon, and Amsaleg]{zhang2020smooth}
Hanwei Zhang, Yannis Avrithis, Teddy Furon, and Laurent Amsaleg.
\newblock Smooth adversarial examples.
\newblock \emph{EURASIP Journal on Information Security}, 2020\penalty0 (1):\penalty0 1--12, 2020{\natexlab{b}}.

\bibitem[Rusu et~al.(2008)Rusu, Marton, Blodow, Dolha, and Beetz]{rusu2008towards}
Radu~Bogdan Rusu, Zoltan~Csaba Marton, Nico Blodow, Mihai Dolha, and Michael Beetz.
\newblock Towards 3d point cloud based object maps for household environments.
\newblock \emph{Robotics and Autonomous Systems}, 56\penalty0 (11):\penalty0 927--941, 2008.

\bibitem[Zhou et~al.(2019)Zhou, Chen, Zhang, Fang, Zhou, and Yu]{zhou2019dup}
Hang Zhou, Kejiang Chen, Weiming Zhang, Han Fang, Wenbo Zhou, and Nenghai Yu.
\newblock Dup-net: Denoiser and upsampler network for 3d adversarial point clouds defense.
\newblock In \emph{Proceedings of the IEEE/CVF International Conference on Computer Vision}, pages 1961--1970, 2019.

\bibitem[Athalye et~al.(2018)Athalye, Carlini, and Wagner]{athalye2018obfuscated}
Anish Athalye, Nicholas Carlini, and David Wagner.
\newblock Obfuscated gradients give a false sense of security: Circumventing defenses to adversarial examples.
\newblock In \emph{International conference on machine learning}, pages 274--283. PMLR, 2018.

\bibitem[Guo et~al.(2019)Guo, Gardner, You, Wilson, and Weinberger]{guo2019simple}
Chuan Guo, Jacob Gardner, Yurong You, Andrew~Gordon Wilson, and Kilian Weinberger.
\newblock Simple black-box adversarial attacks.
\newblock In \emph{International Conference on Machine Learning}, pages 2484--2493. PMLR, 2019.

\bibitem[Yang et~al.(2020)Yang, Jiang, Huang, Ni, and Zhao]{yang2020learning}
Jiancheng Yang, Yangzhou Jiang, Xiaoyang Huang, Bingbing Ni, and Chenglong Zhao.
\newblock Learning black-box attackers with transferable priors and query feedback.
\newblock \emph{Advances in Neural Information Processing Systems}, 33:\penalty0 12288--12299, 2020.

\end{thebibliography}

==> tex/draft.tex <==
\section{Black-box attack}

\begin{algorithm}[t]
\caption{\projabbrv in Black-box setting}
\label{alg:bp-black}
\textbf{Input:} $\cX$: original point cloud to be attacked \\
\textbf{Input:} $t$: true label; $\epsilon_1$ : step size for stage 1; $\epsilon_2$ : step size for stage 2 \\
\textbf{Input:} $\cD$ : a set of imperceptibility regularization\\
\textbf{Input:} $f_s$: surrogate model; $f_b$: target model\\
\textbf{Input:} $\cD$: a set of imperceptibility regularization\\
\textbf{Output:} $\cY^*$
\begin{algorithmic}[1]
\STATE $\cY^* \gets \cX \cdot \mathbf{0}$, $\cY' \gets T_{rsi}(\cX)$
\STATE $\vg \gets \nabla_\cY' {\ell(f_s(T'_{rsi}(\cY')), t)}$
\STATE $\hat{\vg} \gets \func{n}(\vg)$
\STATE $\cS \gets SM(\vg)$ 
\STATE $\cS \gets  Sort(\cS)$
\WHILE{$f_b(T_{rsi}(\cY')) == t$ and $\cS \neq \varnothing$}
    \STATE $\mathbf{s} \gets \cS(0)$
    \STATE $\cS \gets \cS/\mathbf{s}$
    \STATE $\theta \gets \arctan(g_{i2}/g_{i1})$
    \STATE $\mathbf{s} \gets \mathbf{s} \cdot (\cos \theta, \sin \theta, 0)$
    \FOR{$\eta \in \{-\epsilon_1, \epsilon_1\}$}
        \STATE $\cY' \gets \cY' - \eta \vq$
        \IF{$f_b(T'_{rsi}(\cY')) \neq t$}
            \FOR{$D_j \in \cD$}
                \STATE $\hat{\vd_j} \gets \func{n}(\nabla_{\cY'} D_j(\cX,T'_{rsi}(\cY')))$
            \ENDFOR
	\STATE $\{\hat{\vv}_1,\cdots,\hat{\vv}_m\} \gets  GS(\{\hat{\vg},\hat{\vd}_1,\cdots,\hat{\vd}_m\})$ 
            \FOR{$D_j \in \cD$}
            \STATE $\cY' \gets \cY' - \epsilon_2\hat{\vv}_{j}$ 
                % \ENDIF
                \IF{$\sum_j D_{j}(\cX,T'_{rsi}(\cY'))<\sum_j D_{j}(\cX,\cY^*)$}
                \STATE $\cY^* =T'_{rsi}(\cY')$
                \ENDIF
            \ENDFOR
        \ENDIF
    \ENDFOR
\ENDWHILE
    
\end{algorithmic}
\label{alg:black-box}
\end{algorithm}


Here, we provide more details on our black-box attack. As Algorithm \autoref{alg:black-box} shown, given an original point cloud $\cX$, a true label $t$, a set of imperceptibility regularization metrics $\cD$, a black-box model $f_b$ and the surrogate model $f_s$, we calculate the adversarial example $\cY^*$ via a query-based black-box attack. We first estimate the sensitivity map via the gradient of the surrogate model (\cf \emph{Line 4}). Since the sensitivity map is calculated under the coordinate transformation, we denote the coordinate transformation as $T_{rsi}$ and the reverse coordinate transformation as $T'_{rsi}$.
The function $SM(\vg) \defn \{ \mathbf{s}_i\}$, where $\mathbf{s}_i \defn \sqrt{g_{i1}^2 + g_{i2}^2}$. 
$Sort(\cS)$ in \emph{Line 5} means sort all the sensitivity map values of each point descendingly. 
When we do not find an adversarial example for the black-box model and we do not change every point, then we keep searching. At each iteration, we pick the top-ranked value from the sensitivity map $\cS$ as depicted in \emph{Line 7}, \ie $\cS(0)$, and then drop it from $\cS$ (\cf \emph{Line 8}). Similar to our white-box version, at each query step, the algorithm searches along the gradient for misclassification estimated in the surrogate model (\cf \emph{Line 9-12}), and minimizes the distortion along its orthogonal directions while reducing the imperceptibility regularization terms (\cf \emph{Line 13-22}).

In our experimentation, we select a step size of $0.32$ for searching for misclassification, \ie $\epsilon_1 = 0.32$, and $0.16$ for minimizing imperceptibility regularizations, \ie $\epsilon_2 = 0.16$, so that the ASR reaches $100\%$ to ensure a better comparison with other methods. Our method outperforms \siadv in its best parameter. It can be observed in \autoref{fig:abl-black-supp}. The visualization of the black-box attacks is shown in \autoref{fig:vis-3d-blackbox-supp}.

% For a query-based black-box attack, we are provided with an original point cloud $\cX$, a true label t, and a black-box model $f_b$ that allows limited queries. Each query yields output logits representing class probabilities. Our approach begins by leveraging a white-box surrogate model, denoted as $f_s$. The gradients $m_g$ of X are then computed using the sensitivity map~\citep{si_adv_pc}. Similar to the white-box version, each query step involves searching along the gradient for misclassification and minimizing the distortion along its orthogonal directions.
% Within each query step, we employ the gradient direction $\hat g$ derived from mg to conduct a bidirectional search. If the logit decreases, then we orthogonalize $\hat g$ with gradients from various optimization components via the Gram-Schmidt process. In our experimentation, we select a step size of 0.32 for stage 1 and 0.16 for stage 2 so that the ASR reaches 1.0 to ensure a better comparison with other methods. Our method outperforms SI-Adv in its best parameter.






==> tex/related-1.tex <==
\section{Related Work}


\textbf{3D Point Cloud Classification}
(from GSDA)
Early works attempt to classify point clouds by adapting deep learning models in the 2D space ~\cite{su2015multi} \cite{yu2018multi}
In order to directly learn the 3D structure and address the unorderness problem
of point clouds, pioneering methods~\cite{DeepSets} and PointNet~\cite{pointnet} propose
to achieve e nd-to-end learning on point cloud classification by formulating a
general specification. PointNet++~\cite{pointnet++} and other extensive works ~\cite{8953340} \cite{Densepoint} \cite{yang2019modeling} are
built upon PointNet to further capture the fine local structural information from
the neighborhood of each point. Recently, some works focus on either designing
special convolutions on the 3D domain ~\cite{li2018learning} \cite{atzmon2018point} \cite{thomas2019kpconv} \cite{liu2019relation} or developing graph neural
networks ~\cite{simonovsky2017dynamic} \cite{shen2018mining} \cite{dgcnn} \cite{xu2020grid} \cite{Gao_2020_CVPR} to improve point cloud learning. In this paper, we focus on PointNet~\cite{pointnet}, PointNet++~\cite{pointnet++} and DGCNN~\cite{dgcnn} since these models are widely used in 3D point cloud adversarial attacks

%%%%%%%%%%%%%%%%building
\textbf{Adversarial Attack on 3D Point Clouds-}
Deep neural networks are vulnerable to adversarial examples, which have been extensively explored in the field of 2D images. Recently, many early works have applied adversarial attacks to the 3D image domain.Most of the existing 3D point cloud attacks~\cite{origin} ~\cite{wicker2019robustness}~\cite{yang2019adversarial}~\cite{tsai2020robust}~\cite{zheng2019pointcloud}~\cite{zhao2020isometry}~\cite{zhou2020lg}~\cite{hamdi2020advpc}are carried out in the data space, and some of them~\cite{wicker2019robustness}~\cite{yang2019adversarial}~\cite{zheng2019pointcloud} use the method of gradient search.At present, the attacks on the 3D point cloud domain can be mainly divided into two categories: 1) point addition/subtraction attack:Xiang \etal~\cite{origin}proposed point generation attacks by adding a limited number of synthesized points/clusters/objects to a point cloud. 2) point perturbation attack: Early work~\cite{wicker2019robustness}~\cite{yang2019adversarial}~\cite{zheng2019pointcloud} followed the C\&W framework more for point cloud perturbation learning, utilize gradient-guided attack methods to identify critical points from point clouds for deletion.Following the C\&W~\cite{goodfellow2014explaining} framework for point cloud perturbation learning, the 3D coordinates of each point are obtained through end-to-end optimization.Recently,mesh-attack method is proposed to perturb the data grid data.Instead of a 3D adversarial attack that perturbs the point cloud,three mesh losses are adopted, i.e., the chamfer loss to regress the mesh vertices close to their correct position, and the laplacian loss and the edge length loss regularize the mesh to be smoother and avoid the mesh self-intersection and flying vertices problems. 

Although the success rate of the two point cloud attack methods mentioned above is very high, the perturbed point cloud is easily perceived by humans, and some perturbed point clouds will have a large number of outliers or uneven point cloud distribution. situation, this is because the previous work usually did not consider to ensure the geometric characteristics of the point cloud as a whole.
%%%%%%%%%%%%%%%%building(need to add reference)


\textbf{Adversarial Attacks on Shape Invariance in 3D Point Clouds -}

Wen \etal~\cite{geoa3} present an effective algorithm termed Geo+A3-IterNorPro, with Iterative Normal Projection (IterNorPro) that solves a new objective function Geo+A3, Reconstruct the point cloud into a 3D network after the attack, and resample the point cloud from the reconstructed surface grid, while retaining the adversarial effect, successfully deceive the classification model.
 
Hu \etal~\cite{gsda} proposed Graph Spectral Domain Attacks (GSDA) on the basis of Wen \etal~\cite{geoa3} GSDA propose point cloud attacks from a new perspective, aiming to perturb transform coefficients in the graph spectral domain that corresponds to varying certain geometric structure. GSDA adaptively transforms the coordinates of points into the graph domain for compact representation through graph Fourier transform (GFT). The influence of different spectral bands on the point cloud geometry is then analyzed, GFT coefficients in a learnable manner guided by an energy-constrained loss function. Finally, the perturbed graph domain is transformed back to the data domain by inverse GFT (IGFT), generating an adversarial point cloud. The generated point cloud achieves a high attack success rate while maintaining the geometric structure of the point cloud.

Zhang \etal~\cite{mesh-attack} proposed a method called Mesh Attack to directly attack the mesh, sample the results after the Adversarial mesh, and obtain the confrontation point cloud from it.In the early work, KNN-attack and GeoA3 also carried out attacks at the mesh level. Different from Mesh Attack, they first carried out adversarial attacks on the point cloud, and used the mesh reconstructed from the point cloud to carry out adversarial attacks. In GeoA3, this attack is called (pseudo physical scenario attack),
Although GeoA3's attack method at the point cloud level exceeds the KNN attack method, compared with the Mesh Attack method, the attack success rate is reduced by more than 75\% in the pointnet model, and the attack success rate is reduced by more than 90\% in pointnet++

Huang  \etal~\cite{si_adv_pc} proposed a new point cloud sensitivity map to improve the efficiency and unknowability of point cloud perturbation by performing reversible coordinate transformation on the input point cloud to reduce the degree of freedom of points. At the same time, the movement of the point cloud on the tangent plane is limited, and the gradient of the transformed point cloud is obtained on the white box model by using the gradient of the transformed point cloud to calculate the best attack direction. This method greatly reduces the cost of training. On the basis of meeting the shape invariance of the confrontational point cloud, it can also meet the requirements of black box query efficiency

 \paragraph{smooth metrics}

\textbf{Explain what is L2-norm distance, Hausdoff distance, Chamfer distance,Explanation of parameters in the table}:
To achieve imperceptibility, usually introduce L2-norm distance L2~\cite{L2} which measures the square root of the sum of squared shifting distance, Chamfer distance CD ~\cite{CD} which measures the average squared distance between each adversarial point and its nearest original point, Hausdorff distance HD ~\cite{HD} which measures the maximum squared distance between each adversarial point and its nearest original point and is thus sensitive to outliers as the standard of judgment.






